Simulating electronic coherences induced by conical intersections using MASH: Application to attosecond X-ray spectroscopy

In this work, we employ trajectory-based simulations to predict the electronic coherences created by nonadiabatic dynamics near conical intersections. The mapping approach to surface hopping (MASH) is compared with standard fewest-switches surface hopping on three model systems, for which the full quantum-mechanical results are available. Electronic populations and coherences in the adiabatic representation as well as nuclear densities are computed to assess the robustness of the different methods. The results show that standard surface hopping can fail to describe the electronic coherences, whereas they are accurately captured by MASH for the same computational cost. In this way, MASH appears to be an excellent simulation approach for novel X-ray spectroscopies such as the recently proposed Transient Redistribution of Ultrafast Electronic Coherences in Attosecond Raman Signals (TRUECARS).

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
